Snowmass 2021 Instrumentation Frontier (IF5 - MPGDs) -- White Paper 2: Micro Pattern Gaseous Detectors for Nuclear Physics

Many current and future nuclear physics (NP) experiments across the United States have and are implementing micro-pattern gas detectors (MPGDs) to be used for tracking and PID purposes. MPGDs are capable of operating in high rate environments and providing excellent spatial resolution over a large-area with a low material budget. Summarized in this white paper is the role that MPGDs are playing in NP experiments and the R&D which is needed to meet the requirements of future NP experiments.

==> header.tex <==
%%%%%% ``Header'' with a collection of useful definitions  

\RequirePackage{lineno}

\usepackage{graphicx}
%\DeclareGraphicsExtensions{.pdf,.png,.jpg}

\usepackage{url}
\usepackage{hyperref}
\hypersetup{colorlinks=true, linkcolor=black, urlcolor=cyan}
\usepackage[utf8]{inputenc}
%\usepackage[style=numeric-comp,sorting=none]{biblatex}

\usepackage{xspace}

\newcommand{\filenamedot}{.}
\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.1in}
\renewcommand{\topfraction} {0.9}
\renewcommand{\bottomfraction} {0.9}
\renewcommand{\textfraction} {0.1}
\renewcommand{\floatpagefraction} {0.8}

%\usepackage{fancyhdr}
%\pagestyle{fancy}

\usepackage{eurosym}
\usepackage{xcolor}
\usepackage{siunitx}

\newcommand{\hic}{\mbox{$A$$+$$A$}\xspace}
\newcommand{\pA}{\mbox{$p$$+$$A$}\xspace}
\newcommand{\AuAu}{\mbox{Au$+$Au}\xspace}
\newcommand{\auau}{\mbox{Au$+$Au}\xspace} 
\newcommand{\raa}{\mbox{$R_\mathrm{AA}$}\xspace}
\newcommand{\pbpb}{\mbox{Pb$+$Pb}\xspace} 
\newcommand{\pdau}{\mbox{$p(d)$$+$Au}\xspace} 
\newcommand{\pau}{\mbox{$p$$+$Au}\xspace} 
\newcommand{\aj}{\mbox{$A_J$}\xspace} 
\newcommand {\pp}{\mbox{$p$$+$$p$}\xspace}
\newcommand {\ppbar}{\mbox{$p$$+$$\overline{p}$}\xspace}
\newcommand{\pT}{\mbox{${p_T}$}\xspace}
\newcommand{\jpsi}{\mbox{$J/\psi$}}
\newcommand{\sqrtsnn}{\mbox{$\sqrt{s_{\scriptscriptstyle NN}}$}}
\newcommand{\npart}{$N_\mathrm{part}$}
\newcommand{\ncoll}{$N_\mathrm{coll}$}
\newcommand{\qgp}{\mbox{quark-gluon plasma}\xspace}
\newcommand{\jt}{\mbox{$J_T$}} \newcommand{\qhat}{\mbox{$\hat{q}$}}
\newcommand{\Qsqr}{\mbox{$Q^2$}} \newcommand{\CuCu}{\mbox{Cu$+$Cu}}
\newcommand{\PbPb}{\mbox{Pb$+$Pb}} \newcommand{\pPb}{\mbox{$p$$+$Pb}}
\newcommand{\gjet}{\mbox{$\gamma$-jet}}
\newcommand{\Qmax}{\mbox{$Q_{\max}$}} \newcommand{\ET}{\mbox{$E_T$}}
\newcommand{\Et}{\mbox{$E_T$}} \newcommand{\kt}{\mbox{$k_T$}}
\newcommand{\RAA}{\mbox{$R_{AA}$}\xspace} \newcommand{\IAA}{\mbox{$I_{AA}$}}
\newcommand{\pt}{\mbox{${p_T}$}\xspace}
\newcommand{\highpt}{high-${\rm p_{_{T}}}$}
\newcommand{\lessim}{{\stackrel{<}{\sim}}} \newcommand{\eqnpt}{p_T}
\newcommand{\eA}{\mbox{$e-{\rm A}$}}
\newcommand{\dAu}{\mbox{$d$$+$Au}\xspace}
\newcommand{\pAu}{\mbox{$p$$+$Au}\xspace}
\newcommand{\GeVSQ}{\mbox{${\rm GeV}^2$}}
\newcommand{\fastjet}{\mbox{\sc FastJet}\xspace}
\newcommand{\geant}{\mbox{\sc Geant4}\xspace}
\newcommand{\pizero}{\mbox{$\pi^0$}\xspace}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}	 
\newcommand{\green}{\color{green}}	 
\newcommand{\magenta}{\color{magenta}}

\newcommand{\lyxdot}{.}
%\usepackage{subfig}



